Break-for-Make: Modular Low-Rank Adaptations for Composable Content-Style Customization

Personalized generation paradigms empower designers to customize visual intellectual properties with the help of textual descriptions by tuning or adapting pre-trained text-to-image models on a few images. Recent works explore approaches for concurrently customizing both content and detailed visual style appearance. However, these existing approaches often generate images where the content and style are entangled. In this study, we reconsider the customization of content and style concepts from the perspective of parameter space construction. Unlike existing methods that utilize a shared parameter space for content and style, we propose a learning framework that separates the parameter space to facilitate individual learning of content and style, thereby enabling disentangled content and style. To achieve this goal, we introduce "partly learnable projection" (PLP) matrices to separate the original adapters into divided sub-parameter spaces. We propose "break-for-make" customization learning pipeline based on PLP, which is simple yet effective. We break the original adapters into "up projection" and "down projection", train content and style PLPs individually with the guidance of corresponding textual prompts in the separate adapters, and maintain generalization by employing a multi-correspondence projection learning strategy. Based on the adapters broken apart for separate training content and style, we then make the entity parameter space by reconstructing the content and style PLPs matrices, followed by fine-tuning the combined adapter to generate the target object with the desired appearance. Experiments on various styles, including textures, materials, and artistic style, show that our method outperforms state-of-the-art single/multiple concept learning pipelines in terms of content-style-prompt alignment.

==> Figures/task.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{Images/tasks.pdf}
  \caption{
  Comparison of content-style customization task with image stylization and single-content customization. stylization aims at transfer a specific style contained in an image to a new image, without incorporating any edits or regenerating the content of the image. 
  Content-based customization aims to model the content of a given image and generate diverse results for that content based on corresponding prompts. It does so without incorporating customization styles while maintaining a customized content approach.
  content-style customization aims to }
  \label{fig:task}
\end{figure}

==> Sections/intro_bak.tex <==
\section{Introduction}

Text-to-image (T2I) models based on diffusion technology~\cite{ho2020denoising} have demonstrated remarkable proficiency in generating high-quality images, expanding the imaginative powers of the human species through textual descriptions.
Represented by Stable Diffusion~\cite{} and Midjourney~\cite{}, various diffusion models and platforms have been widely applied in the field of creativity design and digital content generation.
Despite the outstanding generalization ability of T2I models, it is challenging for users to generate specific visual concepts using only textual descriptions.

Customized image generation~\cite{hu2021lora,gal2022image,ruiz2023dreambooth,alaluf2023neural} refers to creating diverse images that align with additional content or style images as provided by users. 
However, these approaches tend to model either content or style independently, facing challenges in customized content-style fusion, which represents a specific style within a specific image \cite{zhang2023prospect, shah2023ziplora}.

\input{Figures/task}

Currently, there are primarily two approaches to tackle this challenge. The first approach involves jointly fine-tuning a text-to-image model to simultaneously model both customized content and style \cite{sohn2023styledrop}. 
Alternatively, the second approach involves independently fine-tuning a customized content model and a customized style model in a first stage, and then merging them in the final stage \cite{shah2023ziplora}.
The first method, due to entanglement of content and style during fine-tuning (for example, the intrinsic style of a content image influencing that of a style image), often results in mixture of both during the generation phase. See (a) in Fig.\ref{fig:fig_3_analysis}
In the second method, the merging process often lead to interference between parameters of different models. This oversight can lead to a significant decline in the performance of the merged model, as the integrated parameters may not align optimally, thereby the distinct qualities of both content and style are not preserved effectively after merging\cite{yadav2023resolving}. See (b) in Fig.\ref{fig:fig_3_analysis}.

On the other hand, with the size of pre-trained models increasing in recent years, full fine-tuning – a process that involves retraining all model parameters – has become less feasible due to its time-consuming and resource-intensive nature. 
The method of low-rank parameter adaptation \cite{hu2021lora}has significantly improved the efficiency of fine-tuning processes while still yielding satisfactory results. By fine-tuning these additional adaptations which corresponding to cross-attention parts of diffusion model, rather than the large-sized T2I models, we achieve satisfactory outcomes in terms of both efficiency and effectiveness.

In this work, we propose a parameter separated orthogonal low-rank training method, which achieves customized content-style fusion by training them in separated parameter subspaces of low-rank adaptations independently.
Specifically, we accomplish the separation of content and style parameters by architecting fixed and orthogonal parameter subspaces within low-rank adaptations, which facilitates independent training.
This design of parameter separated training allows the adaptations to effectively disentangle the parameter spaces of style and content. As a result, it preserves the distinct features of both content and style, avoiding conflicts during the generation of images with customized content-style fusion.

Moreover, our separated parameter subspaces approach inherently possesses modular characteristics. This means that the  separately-trained content-style adaptation pair can subsequently be split then combined with other adaptations trained in the same manner (requiring fine-tuning only a few dozen steps). Notably, this process does not necessitate accessing any of the original training information.
This advancement promises significant benefits for the community engaged in text-to-image generation.
Suppose a user has trained a customized content-style adaptation pair and shared it within the community. Other users can then effortlessly break it into content and style components and subsequently combine these with their own corresponding components. This process underpins the rationale behind naming our method \textbf{``break-for-make"}.

Our contributions can be summarized as follows:
\begin{itemize}
\item We have summarized and analyzed the shortcomings, along with the underlying reasons, of the two principal approaches (joint training and merging after training) currently employed in the task of customized content-style image fusion generation.
\item We propose a parameter separated orthogonal low-rank training method,  that effectively achieves the disentanglement of content and style features. This is accomplished by establishing fixed orthogonal parameter groups within the adaptations, which results in the distinct separation of the content parameter space from the style parameter space.
\item The modular nature of our method facilitates the combination of independently trained content and style adaptations. This can be efficiently accomplished with merely a few dozen steps of fine-tuning and notably, does not necessitate access to the original training information.
\item Extensive qualitative and quantitative experiments validate the superior effectiveness of our approach over current baseline methods, particularly in the realms of content and style disentanglement and the preservation of content-style fidelity. Additionally, our method introduces a promising approach for the community to freely combine content and style models easily and efficiently.
\end{itemize}





